On the Throughput Optimization in Large-Scale Batch-Processing Systems

We analyze a data-processing system with $n$ clients producing jobs which are processed in \textit{batches} by $m$ parallel servers; the system throughput critically depends on the batch size and a corresponding sub-additive speedup function. In practice, throughput optimization relies on numerical searches for the optimal batch size, a process that can take up to multiple days in existing commercial systems. In this paper, we model the system in terms of a closed queueing network; a standard Markovian analysis yields the optimal throughput in $\omega\left(n^4\right)$ time. Our main contribution is a mean-field model of the system for the regime where the system size is large. We show that the mean-field model has a unique, globally attractive stationary point which can be found in closed form and which characterizes the asymptotic throughput of the system as a function of the batch size. Using this expression we find the \textit{asymptotically} optimal throughput in $O(1)$ time. Numerical settings from a large commercial system reveal that this asymptotic optimum is accurate in practical finite regimes.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> sections/reviewResponses.tex <==
\section{Response to Reviewer's Comments}
\label{sec:response}
\subsection{Review A} \label{sec:reviewer1}

%Review #53A
\textbf{What area of the paper need improvement?}

The assumption of using at most 3 nodes and 2 job types restricts significance \looseness=-1

\textcolor{brown}{We added Sect. \ref{sec:manyJobManyService} which extends the analysis to multiple job types and multiple levels of service for the case with preemptive priority. We prove global attraction for equal batch sizes and one level of service.}

Lack of comparison with other model classes or existing approximations

\textcolor{brown}{We now briefly discuss the inapplicability of the result from \cite{henderson1990closed} to FCFS scheduling in Sect. \ref{sec:related_work}. A more detailed argument is given below under \emph{Other comments for author}.} 

Technical derivations appear rather standard
%\smallskip

%\textcolor{blue}{(anything reqd?)}

\textbf{Other comments for author}

Generally, I found the paper well-executed, both in the mathematical part, where the derivations have a high level of rigor, and in the experimental part, e.g. D-optimal designs to collect the data.
The authors claim that the class of models is new. They refer in particular to Hendersen et al. in  [19], as a term of comparison. Although they do not fully develop the comparison, which I think they should have done instead, I tend to agree that the model here seems different since the one in [19] supports Poisson distributed batch sizes.
However, works such as [19] have been seminal in developing product-form stochastic Petri nets (SPNs), therefore the authors should look deeper in the literature prior to concluding that their work is entirely original. I believe it is for the dual priority case, since SPNs are not particularly suited to this case, but I have some doubts about the single-class case. In the fluid limit, there is probably little difference between using FCFS scheduling and service in random order, therefore I would expect the model results to match product-form SPNs. I think the authors should develop a full comparison.

\textcolor{brown}{
The main reason for not adopting the framework of Hendeson \etal~ \cite{henderson1990closed} is its inapplicability for FCFS scheduling. For FCFS policy, the position of a job/batch in a node (station) is important and the conditional routing probability $p_j(s_j,a_j)$ in \cite{henderson1990closed} is state dependent. For example, the position of an incoming job in the batching station will depend on the number of existing jobs there. This can be circumvented by using random scheduling as the reviewer commented. However, we chose the fluid approximation over random service order approximation as our framework could then be extended to multiple job types with priority. We have included this discussion under Sect. \ref{sec:related_work} now. Further, a full-fledged comparison with SPNs is beyond the scope of this paper.}

The simulation results are convincing. The real system experimentation is rather narrow. I feel more breadth of systems and problems should be explored. \looseness=-1
%\smallskip

\textcolor{brown}{We provide in this paper simulation as well as real-world experimentation results in a database system. While there are many systems that benefit from batching we opted to concentrate on this specific problem in this paper.}\looseness=-1

My primary concern at the moment is, however, the focus on assuming a small topology as done by the authors. The framework proposed by the authors is based on Kurtz's theorem, which is rather general, therefore I do not see the reason why the framework cannot be extended to an arbitrary number of queues and types. I can see that it may be harder to characterize global attraction, but it seems possible to develop the relevant ODEs. This shortcoming restricts the significance of the paper.

\textcolor{brown}{We have extended the analysis to include the system dynamics for multiple job types and multiple levels of service under preemptive priority in Sect. \ref{sec:manyJobManyService}. We show global attraction, however, only for equal batch size and single level of service.}

\textbf{Other comments: }

Section A.2 is under-developed.
%\textcolor{brown}{We could not provide a detailed analysis of fluid approximation for the non-preemptive case at the moment. However, Fig. \ref{fig:preNpCompare} shows equivalence of preemptive and non-preemptive case when simulated.} 

End of column 2 in page 2. The point about product-forms is not entirely sound. You can efficiently compute throughputs from product forms if you can determine the normalizing constants. You should better say that there aren't methods to do so in [19].

\textcolor{brown}{We have now rephrased the comparison in Sect. \ref{sec:related_work}.}

Typos (not shown here).

\textcolor{brown}{Corrected.}
\vspace{-10pt}
\subsection{Review B} \label{sec:reviewer2}

\textbf{What area of the paper need improvement?}

Model assumptions need to be described better

\smallskip
The manner in which the model scales service rate with batch size is unclear.

\textcolor{brown}{The function which defines the dependence of batch service time (and hence rate) on batch size is termed as \emph{speedup} in our work. In principle, it could be any subadditive function but the exact forms considered for evaluations are described as function $g$ in the second paragraph of Sect.~\ref{subsec:dataFitting}.}

Not sure if the time savings from the approximation are significant for practical ranges of system parameters

\textcolor{brown}{In web applications, handling requests with low latency, is critical, e.g., [X1] reports that the probability of bounces increases by $32\%$ for page-load times of 1 to 3 seconds.
In addition, [X2] reports an empirical increase of performance for every second saved in page-loading time. Works analyzing Amazon shows that a $1\%$ revenue increase is expected for every \SI{100}{\milli\second} of page-load time improvement.
%In turn Amazon loses \SI{1.6}{Billion} \$ per year, for every second of additional page-load.
}

\textcolor{brown}{Keeping such low latency is especially difficult in overload spikes, such as \textit{Black Friday}, \textit{Cyber Monday}, or \textit{Christmas}.}
%E.g., in 2012, Walmart Canada could not handle 6 million page views per minute on \textit{Black Friday}, in consequence their online-store did not respond, causing Walmart to lose real money.
% In the following years, page views per minute even increased:
% Akamai reports 9 million page views per minute on \textit{Black Friday} and 11 million page views per minute on  \textit{Cyber Monday} in 2013 \cite{akamai2013holidayShopping}.
% In 2014, Akamai reports 13 million page views per minute on \textit{Cyber Monday} \cite{akamai2014holidayShopping} and in 2015 the page views per minute almost doubled to 23.5 million for the same event \cite{akamai2015holidayShopping}.
% Unfortunately, we could not get our hands on more recent numbers, but \cite{adobe2020cybermonday, adobe2019ecommerce} report an increase of online sales compared to previous years for 2016 and 2019.}
\textcolor{brown}{As every page view requires to load daily offers, user profiles and preferences, as well as last user transactions, a page view is translated to multiple jobs within the database.
In consequence, the load on the database may be increased by an order of magnitude, compared to the number of requests in the app server.}

\textcolor{brown}{Usually, every request submitted by the application server is executed in a few micro seconds; from our internal measurements, we know that simple jobs run in about \SI{100}{\micro\second}, while jobs consisting of complex calculations run in \SI{300}{\micro\second}.
Obviously, the calculation of a reasonable batch-size has to be processed with a very low execution overhead.
Thus, the time savings from approximation are critical for practical enterprise applications, where an increase of latency results in monetary loss.}

\textcolor{brown}{\noindent[X1] Daniel  An.  2017.Find Out How You Stack Up to New Industry Benchmarks for Mobile Page Speed.  Technical Report. Google Global Product Lead, Mobile Web. 11 pages\newline
[X2] Akamai Technologies Inc. 2017. State  of  Online  Retail  Performance. Technical Report.    Akamai Technologies, Inc. 18 pages.
}
\smallskip

\textbf{Other comments for author}

The paper is written well and addresses an interesting problem. I particularly liked the validation of the analytic technique on a real system. The results look convincing. I suggest the following issues be addressed in the next version.
\smallskip

Real life systems have many features, e.g., queuing for software resources such as buffers/locks, that the current model does not represent. In light of these, the assumptions made need to be better described.

\textcolor{brown}{It is true that certain intricacies of real systems are abstracted away in the model. However, we would like to point out that the results from the prototype system and the model agree for this particular setup as seen in Fig. \ref{fig:others1} and \ref{fig:compareRW}.}

The work seems to assume some kind of linear speedup of service rate with respect to batch size. This needs to be justified. It is also not clear how this speedup is represented in the approximation.

\textcolor{brown}{For analytical derivations, speedup could be any subadditive function to avoid triviality. However, for evaluations, we have experimented with three forms of speedup as described in the second paragraph of Sect. \ref{subsec:dataFitting}. The linear speedup seemed to fit the system data best among these. This was stated clearly in the paper and is specific to the prototype system that we built. Further, the dependence of optimal batch size on the speedup function is shown through the function $\mu(k)$ in \eqref{eq:k_opt}. However, the reviewer is right in pointing out that the argument $k$ has been suppressed in the following sections for brevity.}

The CTMC will give exact solutions in reasonable time if the system is small scale. Would this be sufficient for most real life systems, i.e., is the CTMC enough for most practical ranges of system parameters such as batch size? The paper could perhaps give examples of real systems where application of the CTMC will not be feasible.

\textcolor{brown}{Our experiment results show that the CTMC modeling is accurate. However, the reviewer is right that there are other systems, where batching plays a role, e.g. where service times are heavy-tailed, where the CTMC assumption may not be feasible.}

It will be interesting to see a comparison with simpler models. For example, would an open model simplify the analysis while giving comparable results?

\textcolor{brown}{An open model would not work as the it fails to capture the waiting for response phenomena of the database application. We have actually conducted this analysis and seen that the open model optima are quite far from the behavior of the real system (which is a closed one by construction).}

\vspace{-12pt}
\subsection{Review C} \label{sec:reviewer2}
\textbf{What area of the paper need improvement?}

The analytical techniques applied in the proofs appear to be standard. The proofs of the convergence of the fluid model (ODE) to a unique equilibrium appear to be the most technical part in the proofs, in particular for the two-job type case, but are finally quite straight forward. The proofs of the stochastic convergence are mostly about verifying conditions of existing results from the literature. Also, mean field models have been recently developed and analyzed extensively in various parallel server/queue problems. Thus, from a methodological stand point the contributions are limited.

\textcolor{brown}{We have now included a new result for multiple job types in Sect. \ref{sec:manyJobManyService} where equal batch size and preemptive priority is assumed.}

It is difficult to say if the model is important or relevant from the application context point of view, as this reviewer is not really an expert on performance models for optimizing database queries.

\textcolor{brown}{As mentioned in Sect. \ref{sec:related_work}, batching has drawn attention of the database community quite sometime back \cite{dewitt1984groupcommit} and is still relevant \cite{makreshanski2017batchdb}. Further, our findings are compared against outcomes of experiments done in a commercial system showing the accuracy of the analysis. Please also check a similar remark by Reviewer B.}

The proofs in two job type model need some reworking, in my opinion, see my detailed comments. The result is given for a more general case than the proof currently considers.

\textcolor{brown}{We reworked the proof of Thm. \ref{thm:meanFieldTwoJobs} without assuming $k_1 = k_2$.}

The readability of Section 6 (numerical results) is not that good and there are some minor concerns with figures, see my detailed comments.

\textcolor{brown}{Responses added under detailed comments.}

\textbf{Other comments for author}

p. 3, Section 3: If the number of clients n goes to infinity and the per-client request generation rate $\nu$ goes to zero such that $n*\nu -> \lambda$, wouldn't you get the normal Poisson arrival process and your model would correspond to an open network with a contant arrival rate $\lambda$ in any state? Why not model the system like this? Is the assumption of a finite client population somehow essential?

\textcolor{brown}{In our framework, the per client generation rate is constant. Also, an open network fails to capture the dependence of job arrivals and job completion. We have seen that the optimal batch sizes from an open model and the system do not agree. We opted to show in the paper the appropriate modelling since the system that is used for the experiments is a closed one by construction.}

p. 6: In Theorem 5.1, the proof of the convergence of the ODE and uniqueness of the equilibrium point is only shown for $k_1 = k_2$. The text mentions that the proof for $k_1 \neq k_2$ is exactly the same. However, in my opinion the authors should show this more rigorously than just by stating this claim. Otherwise, the theorem needs to be modified such that it is assumed that $k_1=k_2$, which is anyway assumed later on also in the optimization.

\textcolor{brown}{We reworked the proof of Thm. \ref{thm:meanFieldTwoJobs}. It is now updated for the general case.} \looseness=-1

p. 7, Section 6: What is the role of Section 6.2 and 6.3 for Section 6.4? Sections 6.2/6.3 discuss experimental setup, while 6.4 only uses simulations until the very end shortly in Section 6.4.2, where the experimental work is discussed. Also, presently the experimentation part gets a lot of exposure in terms of text length, but finally there are not that many experiments carried out. It might be better to have a separate section for simulations, i.e., Section 6.1, and then use Section 6.2 for experimentation with all the related text under that subsection.

\textcolor{brown}{We have rearranged Sect. \ref{sec:numerical} as suggested.} 
%\textcolor{brown}{We opted for a storyline that ends now with Sect. 6.2. describing the experimental We use linear speedup of service times in our simulations  Sect. \ref{sec:numerical} as suggested.} 


p. 9, Section 6.4.1: Throughout the section, what is actually meant by simulation? What model is then simulated, the original one obeying (1) or the simplified Markov model? In the text, I assume exact model to mean the numerical solution of the corresponding Markov model and mean field is the fluid model solution.

\textcolor{brown}{The simulation was done as per (1) for the single job type and similarly for two job types. Further, the terms \emph{exact} and \emph{mean field} indeed refer to numerical solution of the steady state equation and the fluid model solution, respectively. We added this clarification to the paper. This is now mentioned towards the beginning of Sect. \ref{sec:numericalEval_}.}

p. 9, Section 6.4.1 (and throughout in Section 6): There is incomplete information on numerical parameters, also service time parameters are not given, constants in linear speed up function not given. Not possible to replicate results.

\textcolor{brown}{Simulation parameters are included towards the beginning of Sect. \ref{sec:numericalEval_}.}

p. 9 Figure 5: In third picture (m=16), the orange exact solution representing the numerical solution for the throughput from the corresponding Markov model has strange non-smooth behavior for n=1000 at k=80 (just before the optimal point). Why is the numerical solution to the Markov model behaving like this? Similar strange behavior can be seen in Figure 6 (c) in the exact solution curves for n=200 with larger batch sizes. Why is the throughput behaving in such jagged, non-smooth manner as a function of the batch size? I could understand if this would be a simulated curve and the simulation time is too short, but the text refers to this as the "exact" result, which I take to mean the numerical solution form the corresponding Markov model.

\textcolor{brown}{The throughput goes down sharply at  points where the number of maximum possible active server drops by one. This becomes even more pronounced as the relative change of the number of active servers increases. For example, for $300$ jobs and $4$ servers, as the batch size increases from $75$  to $76$, the number of maximum possible active servers decreases from $4$ to $3$, causing a sharp drop in the throughput. The reduction is even higher when batch size increases from $100$ to $101$. This is mentioned in Fig. \ref{fig:tPutCompare3} now.}

p. 10, Figure 6: The mean field model does not seem to be very accurate with these values of m and n. How large should the system really be in order to have a better accuracy?

\textcolor{brown}{For the metric we are interested in, which happens to be the optimal batch size/throughput in this system, the mean field model accuracy is reasonable as seen in Fig. \ref{fig:others1} and Fig.~\ref{fig:compareRW}. Note in Fig.~\ref{fig:compareRW} that the batch size is in $\mathbb{N_+}$. The reviewer is correct however in the remark that with a higher number of clients, the mean field model accuracy is expected to be higher.}

p. 10, Figure 7(b): not sure how much information this figure and the test really contains? Why is this important to have?

\textcolor{brown}{This is to explain how quickly the steady-state solution applies to the system.}\looseness=-1

Typos (not shown here).

\textcolor{brown}
{Corrected.}



% \subsection{System with Multiple Job Types and Multiple Levels of Service} \label{sec:multJobsMultService}


% Done except for global attraction.

% \subsection{Comparison with Related Work} \label{sec:compareHenderson}

% Comparison with  \cite{henderson1990closed} included.

% \subsection{Global Attraction for Two Job Types with Different Batch Sizes} \label{sec:globalAttractionK1K2_reply}

% Included in the appendix.

% % \begin{theorem}\label{thm:meanFieldTwoJobsGenl}
% % %\begin{enumerate}[(i)]

% % Consider the transformed stochastic process $z(t)=(z_1(t), z_2(t))$ in Thm. \ref{thm:meanFieldTwoJobs}. Under the assumptions of Thm. \ref{thm:meanFieldTwoJobs}, for any $z_0 \in \{(x_1,x_2): 0 \le x_2 \le x_1 \le 1\}$, we have $z(t) \to z^*$ as $t \to \infty$, where
% % $z^*=(z_1^*,z_2^*)$ is given by:

% % \begin{align*}
% % %\label{eq:fixed_point_two_types_transformed_}
% % z_1^* & = \min (z_{11}^*,z_{12}^*), \\
% % z_2^* &=\eta z_1^*,
% % \end{align*}
% % with 
% % \begin{align*}
% % z_{11}^* & =  \frac{(\mu_1+ \lambda p) \mu_2}{\mu_1  \lambda (1-p)+\mu_2 \lambda p+ \mu_1 \mu_2}, \\
% % z_{12}^* & = \frac{k_1 k_2 (\mu_1+ \lambda p) \mu_2 \alpha}{k_1 \mu_1  \lambda (1-p)+k_2 \mu_2 \lambda p}, \\
% % \eta & = \frac{\lambda p }{\mu_1+ \lambda p}.
% % \end{align*}


% % \end{theorem}
 
% % \begin{proof}
% % We consider following cases:

% % {\bf Case 1}: $k_1 \alpha \geq 1$, $k_2 \alpha \geq 1$\\
% % This case is identical to \textcolor{brown}{Case 1} of Thm. \ref{thm:meanFieldTwoJobs} where the dynamical system is described by a single set of linear equations and convergence to 
% % $(z_{11}^*, \eta z_{11}^*)$ follows.

% % {\bf Case 2}: $k_1 \alpha \geq 1$, $k_2 \alpha < 1$\\
% % If we look at the phase-portrait, we see that the domain of interest is divided into two regions by the line 
% % \begin{align*}
% %  L_1: z_2 &=\frac{k_1}{k_2}(k_2 \alpha -1 + z_1),
% % \end{align*}
% % having respective linear equations. Let us also consider the line
% % \begin{align*}
% %  L_2: z_2 & = \eta z_1.
% % \end{align*}
% % Note that $\dot z_2(t) \ge 0 \iff z$ lies below $L_1$. Thus, if the system starts below $L_1$, it stays there and vice-versa and the fixed point(s) of the system, if exist(s), lie(s) on $L_2$. Let $z_{10}$ denote $z_1$-coordinate of the intersection point of these lines, i.e., 
% % \begin{align*}
% % z_{10} = \frac{k_1 (\mu_1+ \lambda p) (1- k_2 \alpha)}{k_1 \mu_1 +k_1 \lambda p - k_2 \lambda p}.
% % \end{align*}
% % Let us assume 
% % \begin{align*}
% % z_{11}^* \le z_{12}^*.    
% % \end{align*}
% % Calculations show that this implies $z_{10} \le z_{11}^* \le z_{12}^*$. If the system starts from a point below $L_1$, the evolution of the system is given by Eq. \ref{eq:evolutionTwoTypesCase1} and a similar argument as \textcolor{brown}{Case 1} shows that the system converges to the fixed point $(z_{11}^*, \eta z_{11}^*)$. In case the initial point lies above $L_1$, the evolution in the starting phase is given by
% % \begin{align}
% % \label{eq:evolutionTwoTypesCase2New}
% %     \frac{dz_1}{dt}&=-\lambda(1-p)(z_1-z_2)+ k_2 \mu_2(\alpha -\frac{z_2}{k_1}) \nonumber\\
% %     \frac{dz_2}{dt}&=\lambda p(z_1-z_2)-\mu_1z_2
% % \end{align}
% % Calculations show that the real parts of the corresponding eigenvalues are negative and the fixed point for this system is given by $(z_{12}^*, \eta z_{12}^*)$. Thus the system crosses $L_1$ where the evolution is governed by Eq. \ref{eq:evolutionTwoTypesCase1}. From the perspective of convergence, this is equivalent to having the initial point below $L_1$ in which is case the convergence to is already established. Thus, the system always converges to $(z_{11}^*, \eta z_{11}^*)$ when $z_{11}^* \le z_{12}^*$. 

% % For the case
% % \begin{align*}
% % z_{11}^* > z_{12}^*,
% % \end{align*}
% % we notice that $z_{10} \ge z_{11}^* \ge z_{12}^*$ and a similar argument shows convergence of the system to $(z_{12}^*, \eta z_{12}^*)$.

% % {\bf Case 3}: $k_1 \alpha < 1$, $k_2 \alpha < 1$\\
% % When $z_2> k_1 \alpha$, the system evolution is given by Eq. \ref{eq:evolutionTwoTypesCase2Old} and as argued in \textcolor{brown}{Case 2}  of Thm. \ref{thm:meanFieldTwoJobs}, the system eventually reaches a state where $z_2(t) \le k_1 \alpha$. Thus, without loss of generality, we take an initial point satisfying $z_2 \le k_1 \alpha$. 

% % Let us assume
% % \begin{align*}
% % \eta \le k_1 \alpha,
% % \end{align*}
% % Like \textcolor{brown}{Case 2}, we observe that either $z_{10} \le z_{11}^* \le z_{12}^*$ or $z_{10} \ge z_{11}^* \ge z_{12}^*$ and the proof follows the same line of argument as \textcolor{brown}{Case 2}.

% % Now let's consider the scenario when
% % \begin{align*}
% % \eta > k_1 \alpha.
% % \end{align*}
% % We show that $z_{11}^* \ge z_{12}^*$ which holds if and only if
% % \begin{align*}
% % \mu_1 \mu_2 k_1 k_2 \alpha \le k_1 \mu_1  \lambda (1-p) (1- k_2 \alpha) +k_2 \mu_2 \lambda p (1- k_1 \alpha).
% % \end{align*}
% % Since, $\eta > k_1 \alpha$, it suffices to show
% % \begin{align*}
% % \mu_1 \mu_2 k_2 \eta \le k_1 \mu_1  \lambda (1-p) (1- k_2 \alpha) +k_2 \mu_2 \lambda p (1- \eta),
% % \end{align*}
% % which is equivalent to $k_1 (\mu_1 + \lambda p) (1-p) (1- k_2 \alpha) \ge 0$. Similar to \textcolor{brown}{Case 2}, we see that if the initial point lies above $L_1$, the evolution is given by Eq. \ref{eq:evolutionTwoTypesCase2New} and the system converges to $(z_{12}^*, \eta z_{12}^*)$. When started  below $L_1$, the evolution is governed by Eq. \ref{eq:evolutionTwoTypesCase1} initially and the system moves towards $(z_{11}^*, \eta z_{11}^*)$. This eventually changes the evolution dynamics to Eq. \ref{eq:evolutionTwoTypesCase2New} and the system converges to $(z_{12}^*, \eta z_{12}^*)$ in either case.

% % {\bf Case 4}: $k_1 \alpha < 1$, $k_2 \alpha \ge 1$\\
% % Using the same argument as \textcolor{brown}{Case 2}, we take an initial point with $z_2 \le k_1 \alpha$. 

% % Let us first assume
% % \begin{align*}
% % \eta \le k_1 \alpha.
% % \end{align*}
% % Similar to the argument of \textcolor{brown}{Case 3} when $\eta > k_1 \alpha$ and using the fact that $k_2 \alpha \ge 1$, we observe this implies $z_{11}^* \le z_{12}^*$. The convergence from an initial point below or above $L_1$ follows in a similar fashion.

% % The remaining scenario is  
% % \begin{align*}
% % \eta > k_1 \alpha.
% % \end{align*}
% % Similar to \textcolor{brown}{Case 2}, we observe that either $z_{10} \le z_{11}^* \le z_{12}^*$ or $z_{10} \ge z_{11}^* \ge z_{12}^*$ and convergence can be shown to $(z_{11}^*, \eta z_{11}^*)$ or $(z_{12}^*, \eta z_{12}^*)$, respectively, using the same line of argument presented there. 

% % Thus we have established convergence to $(z_{1}^*, \eta z_{1}^*)$ under all scenarios. Note that we have mentioned the actual limit as $(z_{11}^*, \eta z_{11}^*)$ or $(z_{12}^*, \eta z_{12}^*)$, as applicable, in order to be more specific.
% % \end{proof}


% \subsection{Time Saving from Approximation for Practical Cases} \label{sec:timeSaving}

% In web applications, handling requests with low latency, is critical, e.g., \cite{Whitepaper:Delay-Revenue:2017:Google} reports that the probability of bounce increases by $32\%$ for page-load times of 1 to 3 seconds.
% In addition, \cite{Whitepaper:CriticalSecond:2017:Akimai} reports an increase of performance rate by $2\%$ for every second saved in page-loading time for Walmart and $1\%$ revenue increase for Amazon  for every \SI{100}{\milli\second} of page-load time improvement.
% In turn Amazon loses \SI{1.6}{Billion} \$ per year, for every second of additional page-load.

% Keeping such low latency is especially difficult in overload spikes, such as \textit{Black Friday}, \textit{Cyber Monday}, or \textit{Christmas}.
% E.g., in 2012, Walmart Canada could not handle 6 million page views per minute on \textit{Black Friday}, in consequence their online-store did not respond, causing Walmart to lose real money.
% In the following years, page views per minute even increased:
% Akamai reports 9 million page views per minute on \textit{Black Friday} and 11 million page views per minute on  \textit{Cyber Monday} in 2013 \cite{akamai2013holidayShopping}.
% In 2014, Akamai reports 13 million page views per minute on \textit{Cyber Monday} \cite{akamai2014holidayShopping} and in 2015 the page views per minute almost doubled to 23.5 million for the same event \cite{akamai2015holidayShopping}.
% Unfortunately, we could not get our hands on more recent numbers, but \cite{adobe2020cybermonday, adobe2019ecommerce} report an increase of online sales compared to previous years for 2016 and 2019.

% As every page view requires to load daily offers, user profiles and preferences, as well as last user transactions, a page view is translated to multiple jobs within the database.
% In consequence, the load on the database may be increased by an order of magnitude, compared to the number of requests\footnote{i.e., the aforementioned page views per minute} in the app server.

% Usually, every request submitted by the app server is executed in terms of micro seconds; from our internal analysis, we know that simple jobs run in about \SI{100}{\micro\second}, while jobs consisting of complex calculations run in \SI{300}{\micro\second}.
% Obviously, the calculation of a reasonable batch-size has to be processed with an ultra-low execution overhead.
% Thus, the time savings from approximation are critical for practical enterprise applications, where a light amount of additional latency results in heavy monetary loss!

% % {\bf Case 2}: $k_1 \alpha \geq 1$, $k_2 \alpha \le 1$\\
% % If we look at the phase-portrait, we see that the domain of interest is divided into four regions by the lines 
% % \begin{align*}
% %  L_1: z_2 & =\frac{\lambda p }{\mu_1+ \lambda p}z_1,\\
% %  L_2: z_2 &=\frac{k_1}{k_2}(k_2 \alpha -1 + z_1),
% % \end{align*}
% % having respective linear equations. Further, note that $\dot z_2(t) \ge 0 \iff z$ lies below $L_1$. Thus, if the system starts below $L_1$, it stays there and vice-versa. Let $z_{01}$ denote $z_1$-coordinate of the intersection point of these lines, i.e., 
% % \begin{align*}
% % z_{01} = \frac{k_1 (\mu_1+ \lambda p) (1- k_2 \alpha)}{k_1 \mu_1 +k_1 \lambda p - k_2 \lambda p}.
% % \end{align*}
% % Let us assume $z_{11}^* \le z_{12}^*$
